A Visual Programming Paradigm for Abstract Deep Learning Model Development

Deep learning is one of the fastest growing technologies in computer science with a plethora of applications. But this unprecedented growth has so far been limited to the consumption of deep learning experts. The primary challenge being a steep learning curve for learning the programming libraries and the lack of intuitive systems enabling non-experts to consume deep learning. Towards this goal, we study the effectiveness of a no-code paradigm for designing deep learning models. Particularly, a visual drag-and-drop interface is found more efficient when compared with the traditional programming and alternative visual programming paradigms. We conduct user studies of different expertise levels to measure the entry level barrier and the developer load across different programming paradigms. We obtain a System Usability Scale (SUS) of 90 and a NASA Task Load index (TLX) score of 21 for the proposed visual programming compared to 68 and 52, respectively, for the traditional programming methods.

==> 3_system_design_backup.tex <==
\section{Deep Learning IDE (DL-IDE): System Architecture}
\label{system}

(add an introductory paragraph)

\subsection{Language Agnostic Design}
In recent years, there has been rapid progress in the field of Machine Learning, especially Deep Learning. This is accompanied with the development of many libraries which aim to ease the process of constructing a Deep Learning model\footnote{deep learning model, deep neural network, neural network and model are used interchangeably}. Some of the popular and heavily used libraries include Tensorflow~\cite{tensorflow2015-whitepaper}, PyTorch~\cite{paszke2017automatic}, Caffe~\cite{Jia:2014:CCA:2647868.2654889} and Theano~\cite{2016arXiv160502688full}. These and other libraries have their own design and implementation styles which optimize some portion of model construction and/or training. 

The three main phases of building a model are: i) construction, ii) training, and iii) inferencing. As this domain in still in a nascent stage, there are no standard principles which govern these phases. This causes many problems which hinder the productivity of researchers and developers alike. Some of these problems are articulated below:
\begin{itemize}
\item Since there exist multiple languages/libraries and there is no shared standard among them, a model built in one language/library cannot be used or executed from another
\item Due to the previous point, researchers and developers are forced to learn multiple libraries which induces redundancy and increases the learning curve
\item Experimenting and extending openly available models is not possible if the researcher is not familiar with the library in which the model is implemented
\item Adopting a state-of-the-art model to a specific use case is impossible as a developer cannot retrain the model on custom data if the model code is in a library unknown to her
\end{itemize}

To solve these, and other similar problems faced by deep learning researchers, we propose a programming language and library agnostic standard to represent deep learning models. \textbf{Neural Layer Definition Standard (NLDS)} is created to be an industry standard representation of deep neural networks. It aims to bridge the gap between various languages/libraries and provide an intuitive way to design deep learning models. A brief overview of the standard, and an extensive documentation of the same can be found here (link?).

A neural network, as the same suggests, is a network on neurons. A group of neurons form a layer, and multiple layers are stacked on top of each other (with a possibility of skip and recursive connections) to form a deep neural network. Thus NLDS assumes a layer as the fundamental building block of a network. An NLDS definition of an arbitrary neural network contains three parts:
\begin{itemize}
\item Layer definitions - defines the parameters of every layer in the network
\item Link definitions - defines how the layers are connected to each other
\item Hyperparameter definitions - defines model level parameters which define some characteristic properties of the model as a whole
\end{itemize}

These three parts of the NLDS exhaustively captures all aspects of a network's design. Once an NLDS definition is created, it is straight-forward to write transformers which converts the definition into language/library specific executable code. Also, another advantage of NLDS is the following: since we consider layers as the building blocks of a network, and generally a deep network contains not more than several tens of layers, it is feasible to build a UI based network modeler, where a user needs to visually create and connect layers to form a deep learning model. This visual construction, if enabled, will help enhance the productivity of users by eliminating the need to write code.

\subsection{Deep Learning IDE}
Our deep learning IDE supports an intuitive drag-and-drop UI for building deep learning models. The main goals of the framework are:

\begin{itemize}
\item Enabling construction of deep learning models and generation of its code without having to learn specific languages and libraries
\item Have a mechanism to validate the models being constructed so that the errors induced into the architecture are caught during the initial creation phase only and do not leak into the later stages like the training phase where they become difficult to isolate and eliminate and expensive since it consumes GPU resources
\end{itemize}

To achieve these goals, the IDE provides the following features to the users:

\begin{itemize}
\item provides a canvas where users can create layers, configure and connect them to create a deep neural network in a language/library agnostic manner
\item provides real-time validation while the user is constructing the network, thus further increasing the user productivity by catching and eliminating errors during the modelling stage
\item generate and download code for the constructed model in a library of user's choice
\item train the model directly with custom user data and monitor the progress by visualizing metrics of interest
\item deploy the trained model for inferencing (an API endpoint is automatically generated which can be integrated into third-party applications)
\item export the models in  NLDS definition and import/visualize NLDS definitions
\end{itemize}

The below sections describe the internals of the IDE and how NLDS plays a key-role in helping the IDE achieve its goals.

\subsubsection{System Architecture}
The IDE can be divided into four main components: i) user interface, ii) validation service, iii) code generation service, and iv) GPU cluster. It's system architecture is shown in Figure~\ref{fig:sys_arch}.

\begin{figure}
\centering
\includegraphics[scale=0.6]{sys_arch}
\caption{System Architecture}
\label{fig:sys_arch}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\textwidth]{nnm-canvas}
\caption{IDE - UI Canvas}
\label{fig:nnm-canvas}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\textwidth]{nnm-dashboard}
\caption{IDE - UI Dashboard}
\label{fig:nnm-dashboard}
\end{figure}

\begin{itemize}
\item \textbf{User Interface}: The UI contains two sub-components and is the only component with which the user interacts directly. The `Modeler' sub-component provides a canvas for the user to design a network. It also provides a palette of available layers on the left, a section for documentation, validation messages and configuration on the right as shown in Figure~\ref{fig:nnm-canvas}. The `Dashboard' sub-component provides a real-time view of the network's training progress. The user has the freedom to choose the metrics to be plotted as a graph in the dashboard and also to have an overview of the various parameters and hyper-parameters of the training experiment along with visualizing training data as show in Figure~\ref{fig:nnm-dashboard}.

\item \textbf{Validation Service}: The validation service, as the name indicates, validates the model being constructed in the canvas. Each time a change is made to the model, this service is invoked to check the correctness of the model. Any warnings or errors are displayed in the \textit{validation section} of the UI canvas. The user cannot move to a next stage like download, train, etc., if the constructed model is not successfully validated by this service.

\item \textbf{Code Generation Service}: Once the constructed model is validated, the user can either opt to generate and download the source code of the model in a desired library or push the model for training. In both these cases, this component is invoked. In the first case, the code for the model is generated in the library of user's choice and sent back to the canvas for download. In the second case, the model is converted into Tensorflow code and pushed to the GPU cluster for training.

\item \textbf{GPU cluster}: This component can be considered as a plug-gable extension to the IDE and is not one of it's integral part as it can be replaced by any external GPU services like AWS, Google Cloud and IBM Softlayer. The main purpose of this component is to train the model on data provided by the user. The `execution engine' of this component contains GPU hardware and wrappers for low-level firmware like CUDA which come out-of-the-box. The `log manager' is a custom component which continuously watches the training logs for certain metrics identified by the user. These metric values are streamed to the UI dashboard and plotted as graphs. After the training is completed, the trained model is deployed here and an API is exposed to the user for querying.
\end{itemize}

\subsubsection{Data Flow Pipeline}
In this section, we briefly discuss how data flows through IDE. This will also supplement the previous section and provide more details regarding the inner workings of various components. The flow diagram is presented in Figure~\ref{fig:data_pipeline}.

\begin{figure}
\centering
\includegraphics[scale=0.6]{data_pipeline}
\caption{Data Flow Pipeline}
\label{fig:data_pipeline}
\end{figure}

A model being created or modified on the canvas by a user, is internally represented as NLDS by the system. On each change to the model, an NLDS representation reflecting that change is sent to the validation service. This service is embedded with two sets of rules. i) layer level rules - which performs layer level validation and checks each parameter of a layer for value ranges, datatypes, etc., ii) flow level rules - which looks at the connections between the layers and checks for compatibility. It also validates the model-level hyper-parameters. These rule sets are handcrafted by domain experts and enforce the user to follow best practices. If errors are found, the IDs of violated rules, the layers and/or links which violate the rules and user-readable messages are sent back to the UI.

Once the model (NLDS) is validated, it is sent to the code generation service. This service contains transformers, one for each supported library, which convert the NLDS to source code. These transformers contain mappings from NLDS layer definitions to library specific layer code snippets. They also have separate modules which auto-generate code for data pre-processing, model compilation, training and inferencing. The output of this component is well-documented, formatted and readable source code which is then either sent back to the UI for download or sent to the GPU cluster for execution.
    
\begin{comment}
Usage Scenario: 

Motivation: 
    Expert users
    Complexity of dl code

Features: 
\begin{itemize}
\item No code designing 
\item Prevent logical errors (real time static validation) 
\item Platform agnostic code designing 
\end{itemize}
Diagrams and Components:
    model driven development 
    NNM System Diagram 
        User Interface: 
            No code designing 
        Sequence diagram of NNM.
            Use-cases of user interaction    
            Data support
                Text Processing 
                Image Data Processing 
        4 Code generation Microservices:
            -- validation 
                rule book
                types of rule
                    parameters
                    flow validation 
                    
            -- tensorflow/keras
                -- layer types 
            -- Pytorch  
                -- platform specifics 
                
            -- Caffe
                -- protobuf based generation
                
        Types of Users    
            Novice to Experts
            
\end{comment}

==> 6_discussion.tex <==
\section{Discussion}





